Self-attention for raw optical Satellite Time Series Classification

The amount of available Earth observation data has increased dramatically in the recent years. Efficiently making use of the entire body information is a current challenge in remote sensing and demands for light-weight problem-agnostic models that do not require region- or problem-specific expert knowledge. End-to-end trained deep learning models can make use of raw sensory data by learning feature extraction and classification in one step solely from data. Still, many methods proposed in remote sensing research require implicit feature extraction through data preprocessing or explicit design of features. In this work, we compare recent deep learning models on crop type classification on raw and preprocessed Sentinel 2 data. We concentrate on the common neural network architectures for time series, i.e., 1D-convolutions, recurrence, a shallow random forest baseline, and focus on the novel self-attention architecture. Our central findings are that data preprocessing still increased the overall classification performance for all models while the choice of model was less crucial. Self-attention and recurrent neural networks, by their architecture, outperformed convolutional neural networks on raw satellite time series. We explore this by a feature importance analysis based on gradient back-propagation that exploits the differentiable nature of deep learning models. Further, we qualitatively show how self-attention scores focus selectively on few classification-relevant observations.

==> images/confmat/0/isprs_gaf_msresnet/table.tex <==
\begin{tabular}{rlcccc}
\toprule
   &              &  Präzision &       Genauigkeit & $f_1$-score & \#Felder \\
ID & Klasse &            &                   &             &          \\
\midrule
1  & Stilllegungen &      72.85 &             54.58 &       62.40 &      295 \\
2  & Stilllegungen &      98.20 &             98.82 &       98.51 &     7685 \\
3  & Gräser &      82.77 &             81.13 &       81.94 &      906 \\
4  & Gräser &      99.44 &             98.67 &       99.06 &     1807 \\
18 & Winterweizen &      25.00 &              6.06 &        9.76 &       33 \\
19 & Mais &      50.00 &             39.02 &       43.84 &       41 \\
10 & Sommerweizen &      57.63 &             35.05 &       43.59 &       97 \\
11 & Gräser &      77.58 &             95.27 &       85.52 &      719 \\
12 & Gräser &      85.22 &             96.67 &       90.59 &      871 \\
25 & Winterdinkel &      87.18 &             46.36 &       60.53 &      220 \\
27 & Winterroggen &      63.89 &             62.73 &       63.30 &      440 \\
29 & Wintergerste &     100.00 &             83.87 &       91.23 &      248 \\
30 & Sommergerste &       None &              None &        None &     None \\
32 & Sommerhafer &       None &              None &        None &     None \\
53 & Wintertriticale &       None &              None &        None &     None \\
33 & Winterraps &       None &              None &        None &     None \\
56 & Sommerhafer &       None &              None &        None &     None \\
40 & Wintertriticale &       None &              None &        None &     None \\
   &              &            &                   &             &          \\
   & per Klasse &      74.98 &             66.52 &       69.19 &    13362 \\
   &              &            &                   &             &          \\
   & per Parzelle &      kappa &  overall accuracy &             &          \\
   &              &       0.89 &             93.08 &             &          \\
\bottomrule
\end{tabular}



==> images/confmat/0/isprs_gaf_rnn/table.tex <==
\begin{tabular}{rlcccc}
\toprule
   &              &  Präzision &       Genauigkeit & $f_1$-score & \#Felder \\
ID & Klasse &            &                   &             &          \\
\midrule
1  & Stilllegungen &      79.76 &             45.42 &       57.88 &      295 \\
2  & Stilllegungen &      97.34 &             99.56 &       98.44 &     7685 \\
3  & Gräser &      75.96 &             87.20 &       81.19 &      906 \\
4  & Gräser &      98.79 &             99.17 &       98.98 &     1807 \\
18 & Winterweizen &      69.23 &             27.27 &       39.13 &       33 \\
19 & Mais &       0.00 &              0.00 &        0.00 &       41 \\
10 & Sommerweizen &      33.33 &             10.31 &       15.75 &       97 \\
11 & Gräser &      85.07 &             94.30 &       89.45 &      719 \\
12 & Gräser &      86.11 &             92.54 &       89.21 &      871 \\
25 & Winterdinkel &      73.88 &             45.00 &       55.93 &      220 \\
27 & Winterroggen &      62.34 &             44.77 &       52.12 &      440 \\
29 & Wintergerste &      95.93 &             95.16 &       95.55 &      248 \\
30 & Sommergerste &       None &              None &        None &     None \\
32 & Sommerhafer &       None &              None &        None &     None \\
53 & Wintertriticale &       None &              None &        None &     None \\
33 & Winterraps &       None &              None &        None &     None \\
56 & Sommerhafer &       None &              None &        None &     None \\
40 & Wintertriticale &       None &              None &        None &     None \\
   &              &            &                   &             &          \\
   & per Klasse &      71.48 &             61.72 &       64.47 &    13362 \\
   &              &            &                   &             &          \\
   & per Parzelle &      kappa &  overall accuracy &             &          \\
   &              &       0.89 &             92.82 &             &          \\
\bottomrule
\end{tabular}



==> images/confmat/0/isprs_gaf_tempcnn/table.tex <==
\begin{tabular}{rlcccc}
\toprule
   &              &  Präzision &       Genauigkeit & $f_1$-score & \#Felder \\
ID & Klasse &            &                   &             &          \\
\midrule
1  & Stilllegungen &      81.86 &             56.61 &       66.93 &      295 \\
2  & Stilllegungen &      97.79 &             99.64 &       98.70 &     7685 \\
3  & Gräser &      75.21 &             88.74 &       81.42 &      906 \\
4  & Gräser &      99.12 &             99.28 &       99.20 &     1807 \\
18 & Winterweizen &       0.00 &              0.00 &        0.00 &       33 \\
19 & Mais &      42.11 &             19.51 &       26.67 &       41 \\
10 & Sommerweizen &       0.00 &              0.00 &        0.00 &       97 \\
11 & Gräser &      93.26 &             92.35 &       92.80 &      719 \\
12 & Gräser &      87.14 &             94.95 &       90.88 &      871 \\
25 & Winterdinkel &      79.47 &             54.55 &       64.69 &      220 \\
27 & Winterroggen &      62.36 &             51.59 &       56.47 &      440 \\
29 & Wintergerste &      96.43 &             97.98 &       97.20 &      248 \\
30 & Sommergerste &       None &              None &        None &     None \\
32 & Sommerhafer &       None &              None &        None &     None \\
53 & Wintertriticale &       None &              None &        None &     None \\
33 & Winterraps &       None &              None &        None &     None \\
56 & Sommerhafer &       None &              None &        None &     None \\
40 & Wintertriticale &       None &              None &        None &     None \\
   &              &            &                   &             &          \\
   & per Klasse &      67.90 &             62.93 &       64.58 &    13362 \\
   &              &            &                   &             &          \\
   & per Parzelle &      kappa &  overall accuracy &             &          \\
   &              &       0.90 &             93.63 &             &          \\
\bottomrule
\end{tabular}



==> images/confmat/0/isprs_gaf_transformer/table.tex <==
\begin{tabular}{rlcccc}
\toprule
   &              &  Präzision &       Genauigkeit & $f_1$-score & \#Felder \\
ID & Klasse &            &                   &             &          \\
\midrule
1  & Stilllegungen &      72.27 &             58.31 &       64.54 &      295 \\
2  & Stilllegungen &      98.18 &             99.13 &       98.65 &     7685 \\
3  & Gräser &      78.14 &             85.21 &       81.52 &      906 \\
4  & Gräser &      99.28 &             99.17 &       99.22 &     1807 \\
18 & Winterweizen &      69.23 &             27.27 &       39.13 &       33 \\
19 & Mais &      28.00 &             17.07 &       21.21 &       41 \\
10 & Sommerweizen &      40.79 &             31.96 &       35.84 &       97 \\
11 & Gräser &      90.76 &             94.30 &       92.50 &      719 \\
12 & Gräser &      91.45 &             92.08 &       91.76 &      871 \\
25 & Winterdinkel &      69.41 &             69.09 &       69.25 &      220 \\
27 & Winterroggen &      64.40 &             53.86 &       58.66 &      440 \\
29 & Wintergerste &      96.76 &             96.37 &       96.57 &      248 \\
30 & Sommergerste &       None &              None &        None &     None \\
32 & Sommerhafer &       None &              None &        None &     None \\
53 & Wintertriticale &       None &              None &        None &     None \\
33 & Winterraps &       None &              None &        None &     None \\
56 & Sommerhafer &       None &              None &        None &     None \\
40 & Wintertriticale &       None &              None &        None &     None \\
   &              &            &                   &             &          \\
   & per Klasse &      74.89 &             68.65 &       70.74 &    13362 \\
   &              &            &                   &             &          \\
   & per Parzelle &      kappa &  overall accuracy &             &          \\
   &              &       0.90 &             93.62 &             &          \\
\bottomrule
\end{tabular}



==> images/confmat/0/isprs_tum_msresnet/table.tex <==
\begin{tabular}{rlcccc}
\toprule
   &              &  Präzision &       Genauigkeit & $f_1$-score & \#Felder \\
ID & Klasse &            &                   &             &          \\
\midrule
1  & Stilllegungen &      69.33 &             19.45 &       30.38 &      581 \\
2  & Stilllegungen &      89.85 &             98.78 &       94.10 &    10878 \\
3  & Gräser &      67.97 &             73.17 &       70.47 &      995 \\
4  & Gräser &      95.85 &             91.50 &       93.62 &     1917 \\
18 & Winterweizen &       0.00 &              0.00 &        0.00 &       56 \\
19 & Mais &      20.00 &              9.62 &       12.99 &       52 \\
10 & Sommerweizen &       0.00 &              0.00 &        0.00 &      104 \\
11 & Gräser &      77.66 &             67.57 &       72.26 &      777 \\
12 & Gräser &      75.07 &             77.88 &       76.45 &     1017 \\
25 & Winterdinkel &      53.12 &             24.73 &       33.75 &      275 \\
27 & Winterroggen &      43.35 &             22.85 &       29.92 &      499 \\
29 & Wintergerste &      93.70 &             86.77 &       90.10 &      257 \\
30 & Sommergerste &       None &              None &        None &     None \\
32 & Sommerhafer &       None &              None &        None &     None \\
53 & Wintertriticale &       None &              None &        None &     None \\
33 & Winterraps &       None &              None &        None &     None \\
56 & Sommerhafer &       None &              None &        None &     None \\
40 & Wintertriticale &       None &              None &        None &     None \\
   &              &            &                   &             &          \\
   & per Klasse &      57.16 &             47.69 &       50.34 &    17408 \\
   &              &            &                   &             &          \\
   & per Parzelle &      kappa &  overall accuracy &             &          \\
   &              &       0.76 &             86.55 &             &          \\
\bottomrule
\end{tabular}



==> images/confmat/0/isprs_tum_rnn/table.tex <==
\begin{tabular}{rlcccc}
\toprule
   &              &  Präzision &       Genauigkeit & $f_1$-score & \#Felder \\
ID & Klasse &            &                   &             &          \\
\midrule
1  & Stilllegungen &      61.25 &             47.33 &       53.40 &      581 \\
2  & Stilllegungen &      95.79 &             97.33 &       96.56 &    10878 \\
3  & Gräser &      75.74 &             79.70 &       77.67 &      995 \\
4  & Gräser &      94.92 &             97.44 &       96.16 &     1917 \\
18 & Winterweizen &      80.00 &             14.29 &       24.24 &       56 \\
19 & Mais &      41.86 &             34.62 &       37.89 &       52 \\
10 & Sommerweizen &      42.62 &             25.00 &       31.52 &      104 \\
11 & Gräser &      86.38 &             86.49 &       86.43 &      777 \\
12 & Gräser &      82.41 &             89.38 &       85.75 &     1017 \\
25 & Winterdinkel &      65.20 &             48.36 &       55.53 &      275 \\
27 & Winterroggen &      56.11 &             49.70 &       52.71 &      499 \\
29 & Wintergerste &      94.40 &             91.83 &       93.10 &      257 \\
30 & Sommergerste &       None &              None &        None &     None \\
32 & Sommerhafer &       None &              None &        None &     None \\
53 & Wintertriticale &       None &              None &        None &     None \\
33 & Winterraps &       None &              None &        None &     None \\
56 & Sommerhafer &       None &              None &        None &     None \\
40 & Wintertriticale &       None &              None &        None &     None \\
   &              &            &                   &             &          \\
   & per Klasse &      73.06 &             63.46 &       65.91 &    17408 \\
   &              &            &                   &             &          \\
   & per Parzelle &      kappa &  overall accuracy &             &          \\
   &              &       0.84 &             90.61 &             &          \\
\bottomrule
\end{tabular}



==> images/confmat/0/isprs_tum_tempcnn/table.tex <==
\begin{tabular}{rlcccc}
\toprule
   &              &  Präzision &       Genauigkeit & $f_1$-score & \#Felder \\
ID & Klasse &            &                   &             &          \\
\midrule
1  & Stilllegungen &      78.48 &             21.34 &       33.56 &      581 \\
2  & Stilllegungen &      94.07 &             98.12 &       96.05 &    10878 \\
3  & Gräser &      64.09 &             80.90 &       71.52 &      995 \\
4  & Gräser &      94.04 &             96.30 &       95.15 &     1917 \\
18 & Winterweizen &     100.00 &              8.93 &       16.39 &       56 \\
19 & Mais &     100.00 &              1.92 &        3.77 &       52 \\
10 & Sommerweizen &      14.29 &              0.96 &        1.80 &      104 \\
11 & Gräser &      68.36 &             78.12 &       72.91 &      777 \\
12 & Gräser &      71.20 &             86.04 &       77.92 &     1017 \\
25 & Winterdinkel &      61.26 &             24.73 &       35.23 &      275 \\
27 & Winterroggen &      48.17 &             18.44 &       26.67 &      499 \\
29 & Wintergerste &      91.67 &             89.88 &       90.77 &      257 \\
30 & Sommergerste &       None &              None &        None &     None \\
32 & Sommerhafer &       None &              None &        None &     None \\
53 & Wintertriticale &       None &              None &        None &     None \\
33 & Winterraps &       None &              None &        None &     None \\
56 & Sommerhafer &       None &              None &        None &     None \\
40 & Wintertriticale &       None &              None &        None &     None \\
   &              &            &                   &             &          \\
   & per Klasse &      73.80 &             50.47 &       51.81 &    17408 \\
   &              &            &                   &             &          \\
   & per Parzelle &      kappa &  overall accuracy &             &          \\
   &              &       0.79 &             88.06 &             &          \\
\bottomrule
\end{tabular}



==> images/confmat/0/isprs_tum_transformer/table.tex <==
\begin{tabular}{rlcccc}
\toprule
   &              &  Präzision &       Genauigkeit & $f_1$-score & \#Felder \\
ID & Klasse &            &                   &             &          \\
\midrule
1  & Stilllegungen &      51.56 &             56.80 &       54.05 &      581 \\
2  & Stilllegungen &      96.77 &             95.77 &       96.27 &    10878 \\
3  & Gräser &      80.56 &             81.61 &       81.08 &      995 \\
4  & Gräser &      97.74 &             94.89 &       96.29 &     1917 \\
18 & Winterweizen &       0.00 &              0.00 &        0.00 &       56 \\
19 & Mais &      63.64 &             40.38 &       49.41 &       52 \\
10 & Sommerweizen &      60.27 &             42.31 &       49.72 &      104 \\
11 & Gräser &      85.92 &             92.66 &       89.16 &      777 \\
12 & Gräser &      85.69 &             87.71 &       86.69 &     1017 \\
25 & Winterdinkel &      55.03 &             63.64 &       59.02 &      275 \\
27 & Winterroggen &      62.21 &             70.94 &       66.29 &      499 \\
29 & Wintergerste &      93.10 &             94.55 &       93.82 &      257 \\
30 & Sommergerste &       None &              None &        None &     None \\
32 & Sommerhafer &       None &              None &        None &     None \\
53 & Wintertriticale &       None &              None &        None &     None \\
33 & Winterraps &       None &              None &        None &     None \\
56 & Sommerhafer &       None &              None &        None &     None \\
40 & Wintertriticale &       None &              None &        None &     None \\
   &              &            &                   &             &          \\
   & per Klasse &      69.37 &             68.44 &       68.48 &    17408 \\
   &              &            &                   &             &          \\
   & per Parzelle &      kappa &  overall accuracy &             &          \\
   &              &       0.85 &             90.92 &             &          \\
\bottomrule
\end{tabular}



==> images/confmat/1/isprs_gaf_msresnet/table.tex <==
\begin{tabular}{rlcccc}
\toprule
   &              &  Präzision &       Genauigkeit & $f_1$-score & \#Felder \\
ID & Klasse &            &                   &             &          \\
\midrule
1  & Stilllegungen &      74.62 &             65.76 &       69.91 &      295 \\
2  & Stilllegungen &      97.83 &             99.15 &       98.49 &     7685 \\
3  & Gräser &      70.32 &             89.96 &       78.93 &      906 \\
4  & Gräser &      99.44 &             98.89 &       99.17 &     1807 \\
18 & Winterweizen &      16.98 &             27.27 &       20.93 &       33 \\
19 & Mais &      42.86 &             21.95 &       29.03 &       41 \\
10 & Sommerweizen &      49.02 &             25.77 &       33.78 &       97 \\
11 & Gräser &      96.51 &             80.81 &       87.96 &      719 \\
12 & Gräser &      92.54 &             89.78 &       91.14 &      871 \\
25 & Winterdinkel &      75.14 &             63.18 &       68.64 &      220 \\
27 & Winterroggen &      63.67 &             41.82 &       50.48 &      440 \\
29 & Wintergerste &      77.81 &             97.58 &       86.58 &      248 \\
30 & Sommergerste &       None &              None &        None &     None \\
32 & Sommerhafer &       None &              None &        None &     None \\
53 & Wintertriticale &       None &              None &        None &     None \\
33 & Winterraps &       None &              None &        None &     None \\
56 & Sommerhafer &       None &              None &        None &     None \\
40 & Wintertriticale &       None &              None &        None &     None \\
   &              &            &                   &             &          \\
   & per Klasse &      71.39 &             66.83 &       67.92 &    13362 \\
   &              &            &                   &             &          \\
   & per Parzelle &      kappa &  overall accuracy &             &          \\
   &              &       0.88 &             92.70 &             &          \\
\bottomrule
\end{tabular}



==> images/confmat/1/isprs_gaf_rnn/table.tex <==
\begin{tabular}{rlcccc}
\toprule
   &              &  Präzision &       Genauigkeit & $f_1$-score & \#Felder \\
ID & Klasse &            &                   &             &          \\
\midrule
1  & Stilllegungen &      61.67 &             62.71 &       62.18 &      295 \\
2  & Stilllegungen &      97.98 &             98.93 &       98.45 &     7685 \\
3  & Gräser &      70.75 &             87.31 &       78.16 &      906 \\
4  & Gräser &      99.55 &             98.45 &       99.00 &     1807 \\
18 & Winterweizen &       0.00 &              0.00 &        0.00 &       33 \\
19 & Mais &       0.00 &              0.00 &        0.00 &       41 \\
10 & Sommerweizen &       0.00 &              0.00 &        0.00 &       97 \\
11 & Gräser &      91.10 &             89.71 &       90.40 &      719 \\
12 & Gräser &      89.36 &             86.80 &       88.06 &      871 \\
25 & Winterdinkel &      59.05 &             56.36 &       57.67 &      220 \\
27 & Winterroggen &      53.33 &             47.27 &       50.12 &      440 \\
29 & Wintergerste &      95.06 &             93.15 &       94.09 &      248 \\
30 & Sommergerste &       None &              None &        None &     None \\
32 & Sommerhafer &       None &              None &        None &     None \\
53 & Wintertriticale &       None &              None &        None &     None \\
33 & Winterraps &       None &              None &        None &     None \\
56 & Sommerhafer &       None &              None &        None &     None \\
40 & Wintertriticale &       None &              None &        None &     None \\
   &              &            &                   &             &          \\
   & per Klasse &      59.82 &             60.06 &       59.85 &    13362 \\
   &              &            &                   &             &          \\
   & per Parzelle &      kappa &  overall accuracy &             &          \\
   &              &       0.88 &             92.22 &             &          \\
\bottomrule
\end{tabular}



==> images/confmat/1/isprs_gaf_tempcnn/table.tex <==
\begin{tabular}{rlcccc}
\toprule
   &              &  Präzision &       Genauigkeit & $f_1$-score & \#Felder \\
ID & Klasse &            &                   &             &          \\
\midrule
1  & Stilllegungen &      75.45 &             42.71 &       54.55 &      295 \\
2  & Stilllegungen &      97.25 &             99.56 &       98.39 &     7685 \\
3  & Gräser &      64.73 &             85.87 &       73.81 &      906 \\
4  & Gräser &      99.28 &             98.89 &       99.09 &     1807 \\
18 & Winterweizen &       0.00 &              0.00 &        0.00 &       33 \\
19 & Mais &       0.00 &              0.00 &        0.00 &       41 \\
10 & Sommerweizen &       0.00 &              0.00 &        0.00 &       97 \\
11 & Gräser &      73.74 &             83.59 &       78.36 &      719 \\
12 & Gräser &      71.69 &             95.64 &       81.95 &      871 \\
25 & Winterdinkel &      76.04 &             33.18 &       46.20 &      220 \\
27 & Winterroggen &      48.98 &              5.45 &        9.82 &      440 \\
29 & Wintergerste &      98.53 &             81.05 &       88.94 &      248 \\
30 & Sommergerste &       None &              None &        None &     None \\
32 & Sommerhafer &       None &              None &        None &     None \\
53 & Wintertriticale &       None &              None &        None &     None \\
33 & Winterraps &       None &              None &        None &     None \\
56 & Sommerhafer &       None &              None &        None &     None \\
40 & Wintertriticale &       None &              None &        None &     None \\
   &              &            &                   &             &          \\
   & per Klasse &      58.81 &             52.16 &       52.59 &    13362 \\
   &              &            &                   &             &          \\
   & per Parzelle &      kappa &  overall accuracy &             &          \\
   &              &       0.85 &             90.36 &             &          \\
\bottomrule
\end{tabular}



==> images/confmat/1/isprs_gaf_transformer/table.tex <==
\begin{tabular}{rlcccc}
\toprule
   &              &  Präzision &       Genauigkeit & $f_1$-score & \#Felder \\
ID & Klasse &            &                   &             &          \\
\midrule
1  & Stilllegungen &      67.05 &             58.64 &       62.57 &      295 \\
2  & Stilllegungen &      97.84 &             99.14 &       98.49 &     7685 \\
3  & Gräser &      79.24 &             82.56 &       80.86 &      906 \\
4  & Gräser &      99.28 &             99.23 &       99.25 &     1807 \\
18 & Winterweizen &      66.67 &             18.18 &       28.57 &       33 \\
19 & Mais &      27.14 &             46.34 &       34.23 &       41 \\
10 & Sommerweizen &      54.17 &             26.80 &       35.86 &       97 \\
11 & Gräser &      89.97 &             93.60 &       91.75 &      719 \\
12 & Gräser &      93.12 &             90.13 &       91.60 &      871 \\
25 & Winterdinkel &      64.41 &             69.09 &       66.67 &      220 \\
27 & Winterroggen &      60.54 &             50.91 &       55.31 &      440 \\
29 & Wintergerste &      96.71 &             94.76 &       95.72 &      248 \\
30 & Sommergerste &       None &              None &        None &     None \\
32 & Sommerhafer &       None &              None &        None &     None \\
53 & Wintertriticale &       None &              None &        None &     None \\
33 & Winterraps &       None &              None &        None &     None \\
56 & Sommerhafer &       None &              None &        None &     None \\
40 & Wintertriticale &       None &              None &        None &     None \\
   &              &            &                   &             &          \\
   & per Klasse &      74.68 &             69.12 &       70.07 &    13362 \\
   &              &            &                   &             &          \\
   & per Parzelle &      kappa &  overall accuracy &             &          \\
   &              &       0.89 &             93.20 &             &          \\
\bottomrule
\end{tabular}



==> images/confmat/1/isprs_tum_msresnet/table.tex <==
\begin{tabular}{rlcccc}
\toprule
   &              &  Präzision &       Genauigkeit & $f_1$-score & \#Felder \\
ID & Klasse &            &                   &             &          \\
\midrule
1  & Stilllegungen &      45.16 &             55.42 &       49.77 &      581 \\
2  & Stilllegungen &      95.63 &             96.13 &       95.88 &    10878 \\
3  & Gräser &      63.63 &             87.04 &       73.51 &      995 \\
4  & Gräser &      94.77 &             96.35 &       95.55 &     1917 \\
18 & Winterweizen &       0.00 &              0.00 &        0.00 &       56 \\
19 & Mais &      53.85 &             13.46 &       21.54 &       52 \\
10 & Sommerweizen &      50.00 &             18.27 &       26.76 &      104 \\
11 & Gräser &      82.67 &             79.79 &       81.20 &      777 \\
12 & Gräser &      88.65 &             73.75 &       80.52 &     1017 \\
25 & Winterdinkel &      48.31 &             46.91 &       47.60 &      275 \\
27 & Winterroggen &      63.00 &             37.88 &       47.31 &      499 \\
29 & Wintergerste &      97.42 &             88.33 &       92.65 &      257 \\
30 & Sommergerste &       None &              None &        None &     None \\
32 & Sommerhafer &       None &              None &        None &     None \\
53 & Wintertriticale &       None &              None &        None &     None \\
33 & Winterraps &       None &              None &        None &     None \\
56 & Sommerhafer &       None &              None &        None &     None \\
40 & Wintertriticale &       None &              None &        None &     None \\
   &              &            &                   &             &          \\
   & per Klasse &      65.26 &             57.78 &       59.36 &    17408 \\
   &              &            &                   &             &          \\
   & per Parzelle &      kappa &  overall accuracy &             &          \\
   &              &       0.81 &             88.65 &             &          \\
\bottomrule
\end{tabular}



==> images/confmat/1/isprs_tum_rnn/table.tex <==
\begin{tabular}{rlcccc}
\toprule
   &              &  Präzision &       Genauigkeit & $f_1$-score & \#Felder \\
ID & Klasse &            &                   &             &          \\
\midrule
1  & Stilllegungen &      55.92 &             43.89 &       49.18 &      581 \\
2  & Stilllegungen &      95.45 &             97.39 &       96.41 &    10878 \\
3  & Gräser &      73.33 &             81.51 &       77.20 &      995 \\
4  & Gräser &      95.73 &             97.08 &       96.40 &     1917 \\
18 & Winterweizen &      64.29 &             16.07 &       25.71 &       56 \\
19 & Mais &      57.89 &             21.15 &       30.99 &       52 \\
10 & Sommerweizen &      75.61 &             29.81 &       42.76 &      104 \\
11 & Gräser &      89.23 &             85.33 &       87.24 &      777 \\
12 & Gräser &      81.42 &             87.91 &       84.54 &     1017 \\
25 & Winterdinkel &      64.33 &             40.00 &       49.33 &      275 \\
27 & Winterroggen &      55.29 &             51.30 &       53.22 &      499 \\
29 & Wintergerste &      95.28 &             94.16 &       94.72 &      257 \\
30 & Sommergerste &       None &              None &        None &     None \\
32 & Sommerhafer &       None &              None &        None &     None \\
53 & Wintertriticale &       None &              None &        None &     None \\
33 & Winterraps &       None &              None &        None &     None \\
56 & Sommerhafer &       None &              None &        None &     None \\
40 & Wintertriticale &       None &              None &        None &     None \\
   &              &            &                   &             &          \\
   & per Klasse &      75.31 &             62.13 &       65.64 &    17408 \\
   &              &            &                   &             &          \\
   & per Parzelle &      kappa &  overall accuracy &             &          \\
   &              &       0.83 &             90.40 &             &          \\
\bottomrule
\end{tabular}



==> images/confmat/1/isprs_tum_tempcnn/table.tex <==
\begin{tabular}{rlcccc}
\toprule
   &              &  Präzision &       Genauigkeit & $f_1$-score & \#Felder \\
ID & Klasse &            &                   &             &          \\
\midrule
1  & Stilllegungen &       0.00 &              0.00 &        0.00 &      581 \\
2  & Stilllegungen &      86.68 &             98.92 &       92.40 &    10878 \\
3  & Gräser &      50.24 &             53.27 &       51.71 &      995 \\
4  & Gräser &      85.78 &             91.29 &       88.45 &     1917 \\
18 & Winterweizen &       0.00 &              0.00 &        0.00 &       56 \\
19 & Mais &       0.00 &              0.00 &        0.00 &       52 \\
10 & Sommerweizen &       0.00 &              0.00 &        0.00 &      104 \\
11 & Gräser &      51.50 &             48.52 &       49.97 &      777 \\
12 & Gräser &      65.41 &             63.03 &       64.20 &     1017 \\
25 & Winterdinkel &      46.84 &             13.45 &       20.90 &      275 \\
27 & Winterroggen &       0.00 &              0.00 &        0.00 &      499 \\
29 & Wintergerste &     100.00 &             41.63 &       58.79 &      257 \\
30 & Sommergerste &       None &              None &        None &     None \\
32 & Sommerhafer &       None &              None &        None &     None \\
53 & Wintertriticale &       None &              None &        None &     None \\
33 & Winterraps &       None &              None &        None &     None \\
56 & Sommerhafer &       None &              None &        None &     None \\
40 & Wintertriticale &       None &              None &        None &     None \\
   &              &            &                   &             &          \\
   & per Klasse &      40.54 &             34.18 &       35.53 &    17408 \\
   &              &            &                   &             &          \\
   & per Parzelle &      kappa &  overall accuracy &             &          \\
   &              &       0.65 &             81.59 &             &          \\
\bottomrule
\end{tabular}



==> images/confmat/1/isprs_tum_transformer/table.tex <==
\begin{tabular}{rlcccc}
\toprule
   &              &  Präzision &       Genauigkeit & $f_1$-score & \#Felder \\
ID & Klasse &            &                   &             &          \\
\midrule
1  & Stilllegungen &      64.06 &             45.09 &       52.93 &      581 \\
2  & Stilllegungen &      97.23 &             96.10 &       96.66 &    10878 \\
3  & Gräser &      81.50 &             81.91 &       81.70 &      995 \\
4  & Gräser &      93.14 &             97.76 &       95.39 &     1917 \\
18 & Winterweizen &      57.14 &              7.14 &       12.70 &       56 \\
19 & Mais &      37.50 &             46.15 &       41.38 &       52 \\
10 & Sommerweizen &      44.88 &             54.81 &       49.35 &      104 \\
11 & Gräser &      87.71 &             91.89 &       89.75 &      777 \\
12 & Gräser &      83.73 &             89.58 &       86.56 &     1017 \\
25 & Winterdinkel &      50.27 &             68.36 &       57.94 &      275 \\
27 & Winterroggen &      64.94 &             60.12 &       62.43 &      499 \\
29 & Wintergerste &      83.95 &             97.67 &       90.29 &      257 \\
30 & Sommergerste &       None &              None &        None &     None \\
32 & Sommerhafer &       None &              None &        None &     None \\
53 & Wintertriticale &       None &              None &        None &     None \\
33 & Winterraps &       None &              None &        None &     None \\
56 & Sommerhafer &       None &              None &        None &     None \\
40 & Wintertriticale &       None &              None &        None &     None \\
   &              &            &                   &             &          \\
   & per Klasse &      70.50 &             69.72 &       68.09 &    17408 \\
   &              &            &                   &             &          \\
   & per Parzelle &      kappa &  overall accuracy &             &          \\
   &              &       0.85 &             91.07 &             &          \\
\bottomrule
\end{tabular}



==> images/confmat/2/isprs_gaf_msresnet/table.tex <==
\begin{tabular}{rlcccc}
\toprule
   &              &  Präzision &       Genauigkeit & $f_1$-score & \#Felder \\
ID & Klasse &            &                   &             &          \\
\midrule
1  & Stilllegungen &      81.14 &             62.71 &       70.75 &      295 \\
2  & Stilllegungen &      97.90 &             99.41 &       98.65 &     7685 \\
3  & Gräser &      80.74 &             89.29 &       84.80 &      906 \\
4  & Gräser &      99.39 &             99.23 &       99.31 &     1807 \\
18 & Winterweizen &      50.00 &              9.09 &       15.38 &       33 \\
19 & Mais &      53.85 &             51.22 &       52.50 &       41 \\
10 & Sommerweizen &      75.00 &             27.84 &       40.60 &       97 \\
11 & Gräser &      92.52 &             94.58 &       93.54 &      719 \\
12 & Gräser &      92.39 &             94.83 &       93.60 &      871 \\
25 & Winterdinkel &      82.26 &             69.55 &       75.37 &      220 \\
27 & Winterroggen &      70.23 &             61.14 &       65.37 &      440 \\
29 & Wintergerste &      99.59 &             98.39 &       98.99 &      248 \\
30 & Sommergerste &       None &              None &        None &     None \\
32 & Sommerhafer &       None &              None &        None &     None \\
53 & Wintertriticale &       None &              None &        None &     None \\
33 & Winterraps &       None &              None &        None &     None \\
56 & Sommerhafer &       None &              None &        None &     None \\
40 & Wintertriticale &       None &              None &        None &     None \\
   &              &            &                   &             &          \\
   & per Klasse &      81.25 &             71.44 &       74.07 &    13362 \\
   &              &            &                   &             &          \\
   & per Parzelle &      kappa &  overall accuracy &             &          \\
   &              &       0.92 &             94.67 &             &          \\
\bottomrule
\end{tabular}



==> images/confmat/2/isprs_gaf_rnn/table.tex <==
\begin{tabular}{rlcccc}
\toprule
   &              &  Präzision &       Genauigkeit & $f_1$-score & \#Felder \\
ID & Klasse &            &                   &             &          \\
\midrule
1  & Stilllegungen &      75.65 &             49.49 &       59.84 &      295 \\
2  & Stilllegungen &      97.58 &             99.56 &       98.56 &     7685 \\
3  & Gräser &      71.14 &             88.96 &       79.06 &      906 \\
4  & Gräser &      99.01 &             99.34 &       99.17 &     1807 \\
18 & Winterweizen &       0.00 &              0.00 &        0.00 &       33 \\
19 & Mais &     100.00 &              2.44 &        4.76 &       41 \\
10 & Sommerweizen &     100.00 &              1.03 &        2.04 &       97 \\
11 & Gräser &      89.20 &             91.93 &       90.55 &      719 \\
12 & Gräser &      90.09 &             87.72 &       88.89 &      871 \\
25 & Winterdinkel &      58.97 &             62.73 &       60.79 &      220 \\
27 & Winterroggen &      58.55 &             40.45 &       47.85 &      440 \\
29 & Wintergerste &      93.68 &             95.56 &       94.61 &      248 \\
30 & Sommergerste &       None &              None &        None &     None \\
32 & Sommerhafer &       None &              None &        None &     None \\
53 & Wintertriticale &       None &              None &        None &     None \\
33 & Winterraps &       None &              None &        None &     None \\
56 & Sommerhafer &       None &              None &        None &     None \\
40 & Wintertriticale &       None &              None &        None &     None \\
   &              &            &                   &             &          \\
   & per Klasse &      77.82 &             59.93 &       60.51 &    13362 \\
   &              &            &                   &             &          \\
   & per Parzelle &      kappa &  overall accuracy &             &          \\
   &              &       0.88 &             92.64 &             &          \\
\bottomrule
\end{tabular}



==> images/confmat/2/isprs_gaf_tempcnn/table.tex <==
\begin{tabular}{rlcccc}
\toprule
   &              &  Präzision &       Genauigkeit & $f_1$-score & \#Felder \\
ID & Klasse &            &                   &             &          \\
\midrule
1  & Stilllegungen &      77.43 &             67.46 &       72.10 &      295 \\
2  & Stilllegungen &      98.45 &             99.23 &       98.84 &     7685 \\
3  & Gräser &      77.94 &             86.20 &       81.87 &      906 \\
4  & Gräser &      99.45 &             99.39 &       99.42 &     1807 \\
18 & Winterweizen &     100.00 &              3.03 &        5.88 &       33 \\
19 & Mais &      36.84 &             17.07 &       23.33 &       41 \\
10 & Sommerweizen &       0.00 &              0.00 &        0.00 &       97 \\
11 & Gräser &      91.17 &             93.32 &       92.23 &      719 \\
12 & Gräser &      90.43 &             93.34 &       91.86 &      871 \\
25 & Winterdinkel &      71.56 &             68.64 &       70.07 &      220 \\
27 & Winterroggen &      59.13 &             58.86 &       59.00 &      440 \\
29 & Wintergerste &      97.55 &             96.37 &       96.96 &      248 \\
30 & Sommergerste &       None &              None &        None &     None \\
32 & Sommerhafer &       None &              None &        None &     None \\
53 & Wintertriticale &       None &              None &        None &     None \\
33 & Winterraps &       None &              None &        None &     None \\
56 & Sommerhafer &       None &              None &        None &     None \\
40 & Wintertriticale &       None &              None &        None &     None \\
   &              &            &                   &             &          \\
   & per Klasse &      75.00 &             65.24 &       65.96 &    13362 \\
   &              &            &                   &             &          \\
   & per Parzelle &      kappa &  overall accuracy &             &          \\
   &              &       0.90 &             93.87 &             &          \\
\bottomrule
\end{tabular}



==> images/confmat/2/isprs_gaf_transformer/table.tex <==
\begin{tabular}{rlcccc}
\toprule
   &              &  Präzision &       Genauigkeit & $f_1$-score & \#Felder \\
ID & Klasse &            &                   &             &          \\
\midrule
1  & Stilllegungen &      65.81 &             52.20 &       58.22 &      295 \\
2  & Stilllegungen &      98.64 &             98.26 &       98.45 &     7685 \\
3  & Gräser &      77.38 &             81.57 &       79.42 &      906 \\
4  & Gräser &      99.39 &             98.84 &       99.11 &     1807 \\
18 & Winterweizen &      23.08 &             27.27 &       25.00 &       33 \\
19 & Mais &      14.01 &             70.73 &       23.39 &       41 \\
10 & Sommerweizen &      40.00 &              2.06 &        3.92 &       97 \\
11 & Gräser &      94.14 &             87.20 &       90.54 &      719 \\
12 & Gräser &      91.86 &             91.96 &       91.91 &      871 \\
25 & Winterdinkel &      68.91 &             60.45 &       64.41 &      220 \\
27 & Winterroggen &      50.00 &             48.86 &       49.43 &      440 \\
29 & Wintergerste &      79.29 &             98.79 &       87.97 &      248 \\
30 & Sommergerste &       None &              None &        None &     None \\
32 & Sommerhafer &       None &              None &        None &     None \\
53 & Wintertriticale &       None &              None &        None &     None \\
33 & Winterraps &       None &              None &        None &     None \\
56 & Sommerhafer &       None &              None &        None &     None \\
40 & Wintertriticale &       None &              None &        None &     None \\
   &              &            &                   &             &          \\
   & per Klasse &      66.88 &             68.18 &       64.31 &    13362 \\
   &              &            &                   &             &          \\
   & per Parzelle &      kappa &  overall accuracy &             &          \\
   &              &       0.87 &             91.98 &             &          \\
\bottomrule
\end{tabular}



==> images/confmat/2/isprs_tum_msresnet/table.tex <==
\begin{tabular}{rlcccc}
\toprule
   &              &  Präzision &       Genauigkeit & $f_1$-score & \#Felder \\
ID & Klasse &            &                   &             &          \\
\midrule
1  & Stilllegungen &      65.41 &             38.73 &       48.65 &      581 \\
2  & Stilllegungen &      94.67 &             97.67 &       96.15 &    10878 \\
3  & Gräser &      67.61 &             81.81 &       74.03 &      995 \\
4  & Gräser &      97.03 &             93.58 &       95.27 &     1917 \\
18 & Winterweizen &      18.52 &              8.93 &       12.05 &       56 \\
19 & Mais &      33.33 &             15.38 &       21.05 &       52 \\
10 & Sommerweizen &      25.71 &              8.65 &       12.95 &      104 \\
11 & Gräser &      73.98 &             90.73 &       81.50 &      777 \\
12 & Gräser &      80.70 &             84.27 &       82.44 &     1017 \\
25 & Winterdinkel &      65.49 &             26.91 &       38.14 &      275 \\
27 & Winterroggen &      60.48 &             35.27 &       44.56 &      499 \\
29 & Wintergerste &      88.69 &             97.67 &       92.96 &      257 \\
30 & Sommergerste &       None &              None &        None &     None \\
32 & Sommerhafer &       None &              None &        None &     None \\
53 & Wintertriticale &       None &              None &        None &     None \\
33 & Winterraps &       None &              None &        None &     None \\
56 & Sommerhafer &       None &              None &        None &     None \\
40 & Wintertriticale &       None &              None &        None &     None \\
   &              &            &                   &             &          \\
   & per Klasse &      64.30 &             56.63 &       58.31 &    17408 \\
   &              &            &                   &             &          \\
   & per Parzelle &      kappa &  overall accuracy &             &          \\
   &              &       0.81 &             89.29 &             &          \\
\bottomrule
\end{tabular}



==> images/confmat/2/isprs_tum_rnn/table.tex <==
\begin{tabular}{rlcccc}
\toprule
   &              &  Präzision &       Genauigkeit & $f_1$-score & \#Felder \\
ID & Klasse &            &                   &             &          \\
\midrule
1  & Stilllegungen &      61.31 &             42.00 &       49.85 &      581 \\
2  & Stilllegungen &      95.17 &             97.67 &       96.40 &    10878 \\
3  & Gräser &      68.32 &             85.83 &       76.08 &      995 \\
4  & Gräser &      96.11 &             96.56 &       96.33 &     1917 \\
18 & Winterweizen &      71.43 &              8.93 &       15.87 &       56 \\
19 & Mais &      43.48 &             19.23 &       26.67 &       52 \\
10 & Sommerweizen &      65.96 &             29.81 &       41.06 &      104 \\
11 & Gräser &      89.11 &             85.33 &       87.18 &      777 \\
12 & Gräser &      85.48 &             86.23 &       85.85 &     1017 \\
25 & Winterdinkel &      64.71 &             48.00 &       55.11 &      275 \\
27 & Winterroggen &      57.39 &             40.48 &       47.47 &      499 \\
29 & Wintergerste &      92.91 &             96.89 &       94.86 &      257 \\
30 & Sommergerste &       None &              None &        None &     None \\
32 & Sommerhafer &       None &              None &        None &     None \\
53 & Wintertriticale &       None &              None &        None &     None \\
33 & Winterraps &       None &              None &        None &     None \\
56 & Sommerhafer &       None &              None &        None &     None \\
40 & Wintertriticale &       None &              None &        None &     None \\
   &              &            &                   &             &          \\
   & per Klasse &      74.28 &             61.41 &       64.39 &    17408 \\
   &              &            &                   &             &          \\
   & per Parzelle &      kappa &  overall accuracy &             &          \\
   &              &       0.83 &             90.43 &             &          \\
\bottomrule
\end{tabular}



==> images/confmat/2/isprs_tum_tempcnn/table.tex <==
\begin{tabular}{rlcccc}
\toprule
   &              &  Präzision &       Genauigkeit & $f_1$-score & \#Felder \\
ID & Klasse &            &                   &             &          \\
\midrule
1  & Stilllegungen &      71.43 &              0.86 &        1.70 &      581 \\
2  & Stilllegungen &      93.80 &             95.97 &       94.87 &    10878 \\
3  & Gräser &      55.39 &             62.51 &       58.73 &      995 \\
4  & Gräser &      89.10 &             93.79 &       91.39 &     1917 \\
18 & Winterweizen &       0.00 &              0.00 &        0.00 &       56 \\
19 & Mais &       0.00 &              0.00 &        0.00 &       52 \\
10 & Sommerweizen &       0.00 &              0.00 &        0.00 &      104 \\
11 & Gräser &      42.16 &             76.83 &       54.45 &      777 \\
12 & Gräser &      57.88 &             80.14 &       67.22 &     1017 \\
25 & Winterdinkel &      60.00 &             14.18 &       22.94 &      275 \\
27 & Winterroggen &      33.33 &              0.80 &        1.57 &      499 \\
29 & Wintergerste &      84.28 &             75.10 &       79.42 &      257 \\
30 & Sommergerste &       None &              None &        None &     None \\
32 & Sommerhafer &       None &              None &        None &     None \\
53 & Wintertriticale &       None &              None &        None &     None \\
33 & Winterraps &       None &              None &        None &     None \\
56 & Sommerhafer &       None &              None &        None &     None \\
40 & Wintertriticale &       None &              None &        None &     None \\
   &              &            &                   &             &          \\
   & per Klasse &      48.95 &             41.68 &       39.36 &    17408 \\
   &              &            &                   &             &          \\
   & per Parzelle &      kappa &  overall accuracy &             &          \\
   &              &       0.71 &             83.37 &             &          \\
\bottomrule
\end{tabular}



==> images/confmat/2/isprs_tum_transformer/table.tex <==
\begin{tabular}{rlcccc}
\toprule
   &              &  Präzision &       Genauigkeit & $f_1$-score & \#Felder \\
ID & Klasse &            &                   &             &          \\
\midrule
1  & Stilllegungen &      67.90 &             28.40 &       40.05 &      581 \\
2  & Stilllegungen &      94.80 &             97.96 &       96.36 &    10878 \\
3  & Gräser &      71.35 &             80.10 &       75.47 &      995 \\
4  & Gräser &      94.82 &             96.35 &       95.58 &     1917 \\
18 & Winterweizen &       0.00 &              0.00 &        0.00 &       56 \\
19 & Mais &     100.00 &              1.92 &        3.77 &       52 \\
10 & Sommerweizen &      36.36 &             11.54 &       17.52 &      104 \\
11 & Gräser &      86.83 &             85.71 &       86.27 &      777 \\
12 & Gräser &      85.89 &             80.24 &       82.97 &     1017 \\
25 & Winterdinkel &      54.23 &             56.00 &       55.10 &      275 \\
27 & Winterroggen &      53.03 &             61.32 &       56.88 &      499 \\
29 & Wintergerste &      94.76 &             91.44 &       93.07 &      257 \\
30 & Sommergerste &       None &              None &        None &     None \\
32 & Sommerhafer &       None &              None &        None &     None \\
53 & Wintertriticale &       None &              None &        None &     None \\
33 & Winterraps &       None &              None &        None &     None \\
56 & Sommerhafer &       None &              None &        None &     None \\
40 & Wintertriticale &       None &              None &        None &     None \\
   &              &            &                   &             &          \\
   & per Klasse &      70.00 &             57.58 &       58.59 &    17408 \\
   &              &            &                   &             &          \\
   & per Parzelle &      kappa &  overall accuracy &             &          \\
   &              &       0.82 &             89.93 &             &          \\
\bottomrule
\end{tabular}



==> images/models/tsnetransformer <==

	\tikzstyle{conn} = [-stealth, draw=tumblue, rounded corners=1pt]
	\tikzstyle{n} = [circle, inner sep=1pt, fill=tumbluelight]
	\tikzstyle{s} = [tumred]
	\tikzstyle{txtlabel} = [font=\tiny]
	
	
	\newcommand{\attn}{
	\tikzset{external/export next=false}
	\begin{tikzpicture}[yscale=-.4, xscale=.2]
		\node[n](a1) at (-2,0){};
		\node[n](a2) at (-1,0){};
		\node[n](a3) at (0,0){};
		\node[n](a4) at (1,0){};
		\node[n](a5) at (2,0){};
		
		\node[n](b1) at (-2,1){};
		\node[n](b2) at (-1,1){};
		\node[n](b3) at (0,1){};
		\node[n](b4) at (1,1){};
		\node[n](b5) at (2,1){};
		
		\draw[tumred,opacity=.05] (a1) -- (b1);
		\draw[tumred,opacity=.05] (a1) -- (b2);
		\draw[tumred,opacity=.05] (a1) -- (b3);
		\draw[tumred,opacity=.05] (a1) -- (b4);
		\draw[tumred,opacity=.05] (a1) -- (b5);
		\draw[tumred,opacity=.05] (a2) -- (b1);
		\draw[tumred,opacity=.05] (a2) -- (b2);
		\draw[tumred,opacity=.05] (a2) -- (b3);
		\draw[tumred,opacity=.05] (a2) -- (b4);
		\draw[tumred,opacity=.05] (a2) -- (b5);
		\draw[tumred,opacity=.05] (a3) -- (b1);
		\draw[tumred,opacity=.05] (a3) -- (b2);
		\draw[tumred,opacity=.05] (a3) -- (b3);
		\draw[tumred,opacity=.05] (a3) -- (b4);
		\draw[tumred,opacity=.05] (a3) -- (b5);
		
		\draw[tumred,opacity=.8] (a4) -- (b1);
		\draw[tumred,opacity=.8] (a4) -- (b2);
		\draw[tumred,opacity=.8] (a4) -- (b3);
		\draw[tumred,opacity=.8] (a4) -- (b4);
		\draw[tumred,opacity=.8] (a4) -- (b5);
		
		\draw[tumred,opacity=.05] (a5) -- (b1);
		\draw[tumred,opacity=.05] (a5) -- (b2);
		\draw[tumred,opacity=.05] (a5) -- (b3);
		\draw[tumred,opacity=.05] (a5) -- (b4);
		\draw[tumred,opacity=.05] (a5) -- (b5);
		
		%%% HEAD 2
		\draw[tumbluedark,opacity=.8] (a1) -- (b1);
		\draw[tumbluedark,opacity=.8] (a1) -- (b2);
		\draw[tumbluedark,opacity=.8] (a1) -- (b3);
		\draw[tumbluedark,opacity=.8] (a1) -- (b4);
		\draw[tumbluedark,opacity=.8] (a1) -- (b5);
		
		\draw[tumbluedark,opacity=.05] (a2) -- (b1);
		\draw[tumbluedark,opacity=.05] (a2) -- (b2);
		\draw[tumbluedark,opacity=.05] (a2) -- (b3);
		\draw[tumbluedark,opacity=.05] (a2) -- (b4);
		\draw[tumbluedark,opacity=.05] (a2) -- (b5);
		\draw[tumbluedark,opacity=.05] (a3) -- (b1);
		\draw[tumbluedark,opacity=.05] (a3) -- (b2);
		\draw[tumbluedark,opacity=.05] (a3) -- (b3);
		\draw[tumbluedark,opacity=.05] (a3) -- (b4);
		\draw[tumbluedark,opacity=.05] (a3) -- (b5);
		\draw[tumbluedark,opacity=.05] (a4) -- (b1);
		\draw[tumbluedark,opacity=.05] (a4) -- (b2);
		\draw[tumbluedark,opacity=.05] (a4) -- (b3);
		\draw[tumbluedark,opacity=.05] (a4) -- (b4);
		\draw[tumbluedark,opacity=.05] (a4) -- (b5);
		\draw[tumbluedark,opacity=.05] (a5) -- (b1);
		\draw[tumbluedark,opacity=.05] (a5) -- (b2);
		\draw[tumbluedark,opacity=.05] (a5) -- (b3);
		\draw[tumbluedark,opacity=.05] (a5) -- (b4);
		\draw[tumbluedark,opacity=.05] (a5) -- (b5);
		
%		\node[font=\sffamily\tiny] at (0,.5) {self-attention};
		
	\end{tikzpicture}
	}

	\newcommand{\ff}{
		\tikzset{external/export next=false}
		\begin{tikzpicture}[yscale=-.3, xscale=.2]
		\node[n](a1) at (-2,0){};
		\node[n](a2) at (-1,0){};
		\node[n](a3) at (0,0){};
		\node[n](a4) at (1,0){};
		\node[n](a5) at (2,0){};
		
		\node[n](b1) at (-2,1){};
		\node[n](b2) at (-1,1){};
		\node[n](b3) at (0,1){};
		\node[n](b4) at (1,1){};
		\node[n](b5) at (2,1){};
		
		\draw[tumbluelight,-stealth] (a1) -- (b1);
		\draw[tumbluelight,-stealth] (a2) -- (b2);
		\draw[tumbluelight,-stealth] (a3) -- (b3);
		\draw[tumbluelight,-stealth] (a4) -- (b4);
		\draw[tumbluelight,-stealth] (a5) -- (b5);
		
%		\node[font=\sffamily\tiny] at (0,.5) {feed forward};
		\end{tikzpicture}
	}
	
	\newcommand{\block}{
		
	\tikzset{external/export next=false}
	\begin{tikzpicture}[xscale=.5, yscale=-.55]
		\node[inner sep=0](attn) at (0,0){\attn};
		\node[inner sep=0](ff) at (0,1){\ff};
	\end{tikzpicture}
	}
	\tikzset{external/export next=false}
	\begin{tikzpicture}[yscale=-1.2]
	\node(x) at (0,0){\M{X}};{}
	\node[inner sep=0, label={[font=\tiny\sffamily,text width=3em]left:self-attention \\\vspace{2em} feed forward}](l1) at (0,1.2){\block};
	\node[inner sep=0, label={[font=\tiny\sffamily,text width=3em]left:self-attention \\\vspace{2em} feed forward}](l2) at (0,2.4){\block};
	\node[font=\small\sffamily, inner sep=0](a) at (0,3.5){global max-pooling}; %$\text{softmax}(cH)c$ 
	\node[inner sep=0,font=\small\sffamily](s) at (0,4){softmax$(\M{H}\Mweight)$};
	\node[inner sep=0](y) at (0,4.5){\V{y}};
	
	\draw[-stealth, tumbluelight] (x) -- (l1);
	\draw[-stealth, tumbluelight] (l1) -- (l2);
	\draw[-stealth, tumbluelight] (l2) -- (a);
	\draw[-stealth, tumbluelight] (a) -- (s);
	\draw[-stealth, tumbluelight] (s) -- (y);
	\end{tikzpicture}

==> sections/pool.tex <==

\section*{scrap Material...}


\section*{Data preprocessing and End-to-End Learning}
A common assumption in Remote sensing is that data preprocessing is a necessity for accurate classification on satellite time series:
Atmospheric correction is used to translate top-of-atmosphere to bottom-of-atmosphere reflectances using a predefined functional model of the radiometric transfer of the energy through the atmosphere \citep{}.   
Classification models are employed to identify pixels covered by snow, clouds or cloudshadow \citep{} through existing models like Fmask \citep{}, Maja \citep{}, or pretrained Convolutional Neural Networks \citep{}.
With these noisy pixels identified, a temporal interpolation can be applied to \textsl{fill the gaps} \citep{}.
All of these preprocessing steps can be conceptually summarized into a preprocessing function $f_{\Mweight_\text{preproc}}$ that is parameterized $\Mweight_\text{prproc}$ by previously determined or hand-picked model parameters for atmospheric correction, cloud tolerance thresholds, or start and end-dates for the selection of suitable timespan of a certain application.   

The preprocessed signal, however, is usually only an intermediate product. 
Today, a final application is commonly obtained via a deep learning model $f_\Mweight$ that approximates a mapping from an input domain $\M{X}$ to a target domain $\V{y}$. 
Deep learning models are implemented by cascaded neural network layers that form a problem-agnostic, non-linear differentiable function.
The parameters $\Mweight$ are determined by the minimization $\min_{\Mweight} \mathcal{L}(\V{y},f_{\Mweight}(\M{X}))$ of an objective function $\mathcal{L}$ between ground truth $\V{y}$ and approximation $\yhat = f_{\Mweight}(\M{X})$.
The objective function is minimized via stochastic gradient descent $\Mweight \leftarrow \Mweight - \lr\frac{\partial\mathcal{L}}{\partial\Mweight}$ that iteratively updates the parameters scaled by their influence on the loss function through backpropagated gradients $\frac{\partial\mathcal{L}}{\partial\Mweight}$.
This optimization guarantees that the chosen paramters $\Mweight$ are optimal with respect to the observed dataset and objective function.

In contrast, the parameters of the preprocesing function $\Mweight_\text{preproc}$ are determined based on task and region specific expert knowledge that often boils down to best practices and prior region or data-specific experience of the model designer. 
There are no guarantees the preprocessing parameters are optimal for a specific task. Further is is unclear if data preprocessing procedures are even necessary for particular application.
%Hence, we argue that data preprocessing and end-to-end optimization follow two orthogonal paradigms that are not compatible.

In this work, we empirically question the necessity of time series preprocessing on a classification task of vegetation types when sufficient data is available. 
We show quantitative results comparing state-of-the-art time series classification models on preprocessed and raw Sentinel 2 data and qualitatively investigate the mechanisms that allow some models to cope with raw satellite data.

%Network hyper-parameters related to the particular neural network architecture and optimization technique are chosen based on an increasingly abstract 

%\begin{figure}
%	\input{images/preprocessing.tikz}
%\end{figure}

\begin{figure}
	\centering\input{images/preprocessing_and_end2end.tikz}
	\caption{Schematic illustration of the training of end-to-end trainable neural network $f_{\Mweight}$ on raw data $\M{X}$ with a preprocessing function $f_{\Mweight_\text{preproc}}$.%
		The neural network $f_\Mweight$ paramters $\Mweight$ are optimized via gradient backpropagation and are guaranteed to be locally optimal with respect to dataset and loss function. 
		In contrast, the parameters of the preprocessing function are often defined based on region-specific expert knowledge without any guarantee of optimiality. 
	}
\end{figure}


\subsection{Class-wise accuracy}
\begin{figure}
	\input{images/confmat.tikz}
	
	\def\id{2}
	
	\begin{subfigure}{.245\textwidth}
		%	\tikzsetnextfilename{}
		\confmat{images/confmat/0/isprs_gaf_rnn/confmat_flat.csv}
	\end{subfigure}
	\begin{subfigure}{.245\textwidth}
		\confmat{images/confmat/0/isprs_gaf_transformer/confmat_flat.csv}
	\end{subfigure}
	\begin{subfigure}{.245\textwidth}
		\confmat{images/confmat/1/isprs_gaf_msresnet/confmat_flat.csv}
	\end{subfigure}
	\begin{subfigure}{.245\textwidth}
		\confmat{images/confmat/1/isprs_gaf_tempcnn/confmat_flat.csv}
	\end{subfigure}
	
	\begin{subfigure}{.245\textwidth}
		\confmat{images/confmat/0/isprs_tum_rnn/confmat_flat.csv}
	\end{subfigure}
	\begin{subfigure}{.245\textwidth}
		\confmat{images/confmat/1/isprs_tum_transformer/confmat_flat.csv}
	\end{subfigure}
	\begin{subfigure}{.245\textwidth}
		\confmat{images/confmat/0/isprs_tum_msresnet/confmat_flat.csv}
	\end{subfigure}
	\begin{subfigure}{.245\textwidth}
		\confmat{images/confmat/2/isprs_tum_tempcnn/confmat_flat.csv}
	\end{subfigure}
	
	\caption{s}
\end{figure}

\subsection{More raw data versus few Preprocessed}
\label{sec:exp:quantitative:sel}

The previous experiment evaluated the model performances the identical training examples on preprocessed and raw data on all available regions: Hollfeld, Krumbach and Bavarian Forest.
The quantity of the examples were identifical for both preprocessed and raw datasets.
In this experiment we vary the size of the datasets and observe if the model performance would benefit from a larger body of training data, even if the additional samples are from a spatially distant region.
This is a realisic scenario, since preprocessed data may be only available at a small quantity due to the computational requirements and the partial supervision of the model designer. 

In \cref{tab:hollkrum}, we show results this property in two configurations.
\Cref{tab:holl:kappa,tab:holl:accuracy} show accuracy and kappa metrics from the evaluation partition of the Hollfeld partition. 
The first row shows the performance of the models on preprocessed data trained solely on the Hollfeld partition.
In the second and third rows show models trained on raw dataset either on the entire dataset or only on the Hollfeld partition.
In \cref{tab:krum:kappa,tab:krum:accuracy} we repeat this experiment with evaluating on Krumbach. 
We show results from the 23 class configurations, as we consider this the more challenging tasks for the neural networks.

{\Large \textbf{TODO DETAILED DESCRIPTION}}


\begin{table}
	\vspace{1em}
	\begin{subtable}{\textwidth}
		\centering\input{tables/holl/kappa.tex}
		\caption{Kappa Metric 23 classes}
		\label{tab:holl:kappa}
	\end{subtable}
	
	\vspace{1em}
	\begin{subtable}{\textwidth}
		\centering\input{tables/holl/accuracy.tex}
		\caption{Overall Accuracy 23 classes}
		\label{tab:holl:accuracy}
	\end{subtable}
	
	%	\begin{subtable}{\textwidth}
	%	\caption{Kappa Metric 12 classes}
	%	\label{tab:holl2:kappa}
	%	%\centering\input{tables/holl2/kappa.tex}
	%	\end{subtable}
	%	
	%	\vspace{1em}
	%	\begin{subtable}{\textwidth}
	%		\caption{Overall Accuracy 12 classes}
	%		\label{tab:holl2:accuracy}
	%		%\centering\input{tables/holl2/accuracy.tex}
	%	\end{subtable}
	%\end{table}
	%
	%\begin{table}
	\vspace{1em}
	\begin{subtable}{\textwidth}
		\centering\input{tables/krum/kappa.tex}
		\caption{Kappa Metric 23 classes}
		\label{tab:krum:kappa}
	\end{subtable}
	
	\vspace{1em}
	\begin{subtable}{\textwidth}
		\centering\input{tables/krum/accuracy.tex}
		\caption{Overall Accuracy 23 classes}
		\label{tab:krum:accuracy}
	\end{subtable}
	
	%	\vspace{1em}
	%	\begin{subtable}{\textwidth}
	%		\caption{Kappa Metric 12 classes}
	%		\label{tab:krum2:kappa}
	%		\centering\input{tables/krum2/kappa.tex}
	%	\end{subtable}
	%	
	%	\vspace{1em}
	%	\begin{subtable}{\textwidth}
	%		\caption{Overall Accuracy 12 classes}
	%		\label{tab:krum2:accuracy}
	%		\centering\input{tables/krum2/accuracy.tex}
	%	\end{subtable}
	
	\caption{Evaluation of the benefit of inclusion of data for spatially distant regions for classification}
	\label{tab:hollkrum}
	
\end{table}


==> tables/holl/accuracy.tex <==
\begin{tabular}{lllcccc}
\toprule
kappa & trained on & tested on & \rnn & \transformer & \msresnet & \tempcnn \\
\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}
    	processed & Hollfeld & Hollfeld & 0.80$^{\pm0.00}$ & 0.81$^{\pm0.00}$ & 0.83$^{\pm0.01}$ & 0.83$^{\pm0.00}$ \\ 
	raw       & Hollfeld+Krumbach+Bav.Forest & Hollfeld & 0.74$^{\pm0.04}$ & 0.78$^{\pm0.01}$ & 0.75$^{\pm0.00}$ & 0.73$^{\pm0.01}$ \\ 
	raw       & Hollfeld & Hollfeld & 0.74$^{\pm0.01}$ & 0.73$^{\pm0.04}$ & 0.75$^{\pm0.00}$ & 0.73$^{\pm0.01}$ \\ 
\bottomrule
\end{tabular}


==> tables/holl/holl_accuracy.tex <==
%\renewcommand{\arraystretch}{.8}
%\setlength\tabcolsep{0pt}
\begin{tabular}{lcccccc}
	\toprule
	ov. acc. & \svm & \rf & \rnn & \transformer & \msresnet & \tempcnn \\
	\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}
pre (holl) & & & 0.81$^{\pm0.01}$ & 0.81$^{\pm0.01}$ & 0.83$^{\pm0.02}$ & 0.83$^{\pm0.00}$ \\ 
raw (all) & & & 0.57$^{\pm0.28}$ & 0.78$^{\pm0.03}$ & 0.75$^{\pm0.01}$ & 0.73$^{\pm0.02}$ \\ 
raw (holl) & & & 0.57$^{\pm0.27}$ & 0.74$^{\pm0.08}$ & 0.73$^{\pm0.00}$ & 0.70$^{\pm0.08}$ \\ 
	\bottomrule
\end{tabular}

==> tables/holl/holl_kappa.tex <==
%\renewcommand{\arraystretch}{.8}
%\setlength\tabcolsep{0pt}
\begin{tabular}{lcccccc}
	\toprule
	ov. acc. & \svm & \rf & \rnn & \transformer & \msresnet & \tempcnn \\
	\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}
pre (holl) & & & 0.75$^{\pm0.01}$ & 0.76$^{\pm0.01}$ & 0.78$^{\pm0.03}$ & 0.78$^{\pm0.00}$ \\ 
raw (all) & & & 0.22$^{\pm0.63}$ & 0.70$^{\pm0.04}$ & 0.66$^{\pm0.00}$ & 0.62$^{\pm0.03}$ \\ 
raw (holl) & & & 0.22$^{\pm0.62}$ & 0.64$^{\pm0.12}$ & 0.63$^{\pm0.00}$ & 0.57$^{\pm0.14}$ \\ 
	\bottomrule
\end{tabular}

==> tables/holl/kappa.tex <==
\begin{tabular}{lllcccc}
\toprule
ov.acc & trained on & tested on & \rnn & \transformer & \msresnet & \tempcnn \\
\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}
    	processed & Hollfeld & Hollfeld & 0.74$^{\pm0.00}$ & 0.76$^{\pm0.01}$ & 0.78$^{\pm0.01}$ & 0.78$^{\pm0.00}$ \\ 
	raw       & Hollfeld+Krumbach+Bav.Forest & Hollfeld & 0.63$^{\pm0.06}$ & 0.70$^{\pm0.02}$ & 0.66$^{\pm0.00}$ & 0.62$^{\pm0.02}$ \\ 
	raw       & Hollfeld & Hollfeld & 0.64$^{\pm0.02}$ & 0.64$^{\pm0.06}$ & 0.66$^{\pm0.00}$ & 0.62$^{\pm0.01}$ \\ 
\bottomrule
\end{tabular}


==> tables/krum/accuracy.tex <==
\begin{tabular}{lllcccc}
\toprule
ov.acc & trained on & tested on & \rnn & \transformer & \msresnet & \tempcnn \\
\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}
    	processed & Krumbach & Krumbach & 0.92$^{\pm0.00}$ & 0.92$^{\pm0.00}$ & 0.93$^{\pm0.01}$ & 0.93$^{\pm0.01}$ \\ 
	raw       & Krumbach+Hollfeld+Bav.Forest & Krumbach & 0.88$^{\pm0.00}$ & 0.85$^{\pm0.03}$ & 0.88$^{\pm0.00}$ & 0.85$^{\pm0.02}$ \\ 
	raw       & Krumbach & Krumbach & 0.88$^{\pm0.00}$ & 0.87$^{\pm0.03}$ & 0.87$^{\pm0.00}$ & 0.87$^{\pm0.00}$ \\ 
\bottomrule
\end{tabular}


==> tables/krum/kappa.tex <==
\begin{tabular}{lllcccc}
\toprule
kappa & trained on & tested on & \rnn & \transformer & \msresnet & \tempcnn \\
\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}
    	processed & Krumbach & Krumbach & 0.87$^{\pm0.01}$ & 0.89$^{\pm0.01}$ & 0.90$^{\pm0.01}$ & 0.89$^{\pm0.01}$ \\ 
	raw       & Krumbach+Hollfeld+Bav.Forest & Krumbach & 0.81$^{\pm0.00}$ & 0.77$^{\pm0.05}$ & 0.81$^{\pm0.00}$ & 0.77$^{\pm0.03}$ \\ 
	raw       & Krumbach & Krumbach & 0.81$^{\pm0.00}$ & 0.79$^{\pm0.05}$ & 0.80$^{\pm0.00}$ & 0.80$^{\pm0.01}$ \\ 
\bottomrule
\end{tabular}


==> tables/krum/krum_accuracy.tex <==
%\renewcommand{\arraystretch}{.8}
%\setlength\tabcolsep{0pt}
\begin{tabular}{lcccc}
	\toprule
	ov. acc.\rnn & \transformer & \msresnet & \tempcnn \\
	\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}
	\bottomrule
\end{tabular}

==> tables/krum/krum_kappa.tex <==
%\renewcommand{\arraystretch}{.8}
%\setlength\tabcolsep{0pt}
\begin{tabular}{lcccccc}
	\toprule
	ov. acc. & \svm & \rf & \rnn & \transformer & \msresnet & \tempcnn \\
	\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}
pre (holl) & & & 0.75$^{\pm0.01}$ & 0.76$^{\pm0.01}$ & 0.78$^{\pm0.03}$ & 0.78$^{\pm0.00}$ \\ 
raw (all) & & & 0.22$^{\pm0.63}$ & 0.70$^{\pm0.04}$ & 0.66$^{\pm0.00}$ & 0.62$^{\pm0.03}$ \\ 
raw (holl) & & & 0.22$^{\pm0.62}$ & 0.64$^{\pm0.12}$ & 0.63$^{\pm0.00}$ & 0.57$^{\pm0.14}$ \\ 
	\bottomrule
\end{tabular}

==> tables/krum2/accuracy.tex <==
\begin{tabular}{lcccc}
\toprule
ov.acc & \rnn & \transformer & \msresnet & \tempcnn \\
\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}
    	pre (holl) & 0.96$^{\pm0.00}$ & 0.96$^{\pm0.01}$ & 0.97$^{\pm0.00}$ & 0.97$^{\pm0.00}$ \\ 
	raw (all) & 0.94$^{\pm0.00}$ & 0.95$^{\pm0.00}$ & 0.94$^{\pm0.00}$ & 0.92$^{\pm0.02}$ \\ 
	raw (holl) & 0.94$^{\pm0.00}$ & 0.92$^{\pm0.03}$ & 0.93$^{\pm0.00}$ & 0.91$^{\pm0.02}$ \\ 
\bottomrule
\end{tabular}


==> tables/krum2/kappa.tex <==
\begin{tabular}{lcccc}
\toprule
kappa & \rnn & \transformer & \msresnet & \tempcnn \\
\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}
    	pre (holl) & 0.93$^{\pm0.00}$ & 0.94$^{\pm0.02}$ & 0.96$^{\pm0.00}$ & 0.96$^{\pm0.00}$ \\ 
	raw (all) & 0.89$^{\pm0.00}$ & 0.91$^{\pm0.01}$ & 0.89$^{\pm0.00}$ & 0.86$^{\pm0.04}$ \\ 
	raw (holl) & 0.89$^{\pm0.01}$ & 0.85$^{\pm0.05}$ & 0.88$^{\pm0.01}$ & 0.84$^{\pm0.03}$ \\ 
\bottomrule
\end{tabular}


==> tables/preraw.old.tex <==
	\small
\renewcommand{\arraystretch}{.8}
\setlength\tabcolsep{0pt}
\caption{Kappa metric and overall accuracy of the deep learning model on preprocessed and raw datasets.}
\label{tab:accuracy}
\begin{tabular}{rcccccccccc}
	\toprule
	& \multicolumn{2}{c}{RNN (LSTM)$^2$} & \multicolumn{2}{c}{Transformer$^3$} & \multicolumn{2}{c}{MS-ResNet$^1$} & \multicolumn{2}{c}{TempCNN$^4$} \\
	layer & \multicolumn{2}{c}{recurrence} & \multicolumn{2}{c}{self-attention} & \multicolumn{2}{c}{convolution} & \multicolumn{2}{c}{convolution} \\
	param. & \multicolumn{2}{c}{100k} & \multicolumn{2}{c}{600k} & \multicolumn{2}{c}{2M} & \multicolumn{2}{c}{433k} \\
	\midrule
	& $\kappa$-metric & accuracy & $\kappa$-metric & accuracy & $\kappa$-metric & accuracy &  $\kappa$-metric & accuracy \\ 
	\cmidrule(lr){2-3}\cmidrule(lr){4-5} \cmidrule(lr){6-7}\cmidrule(lr){8-9}
	prepr. & \textbf{.759} $^{\pm .0037}$ & \textbf{.804} $^{\pm.0031}$ & .759 $^{\pm .0017}$ & .804 $^{\pm.0011}$ & \textbf{.816} $^{\pm .0048}$ & \textbf{.849}$^{\pm .0041}$ & \textbf{.799} $^{\pm .0015}$ & \textbf{.836} $^{\pm .0012}$ \\
	raw & .756 $^{\pm .0037}$ & .801 $^{\pm .0026}$ & \textbf{.808} $^{\pm .0052}$ & \textbf{.842} $^{\pm .0043}$ & .800 $^{\pm .0039}$ & {.836} $^{\pm .0033}$ & .750 $^{\pm .0036}$ & .799 $^{\pm .0027}$ \\
	\midrule
	$\Delta$ & .003 $^{\pm .0048}$ & .003 $^{\pm .0041}$ & -.049 $^{\pm .0054}$ & -.038 $^{\pm .0045}$ & .016 $^{\pm .0060}$ & .013 $^{\pm .0055}$ & .049 $^{\pm .0036}$ & .038 $^{\pm .0029}$ \\
	\bottomrule
\end{tabular}

==> tables/preraw.tex <==
\small
%\renewcommand{\arraystretch}{.8}
%\setlength\tabcolsep{0pt}
\caption{Kappa metric and overall accuracy of the deep learning model on preprocessed and raw datasets.}
\label{tab:accuracy}
\begin{tabular}{rcccccc}
	\toprule
	kappa & svm & rf & rnn & transformer & msresnet & tempcnn \\
	pre & & & 0.79$^{\pm0.00}$ & 0.81$^{\pm0.01}$ & 0.82$^{\pm0.02}$ & 0.81$^{\pm0.01}$ \\
	raw & & & 0.72$^{\pm0.01}$ & 0.74$^{\pm0.03}$ & 0.72$^{\pm0.01}$ & 0.68$^{\pm0.02}$ \\
	\bottomrule
\end{tabular}

==> tables/preraw2_accuracy.tex <==
%\renewcommand{\arraystretch}{.8}
%\setlength\tabcolsep{0pt}
\begin{tabular}{lcccccc}
	\toprule
	ov. acc. & \svm & \rf & \rnn & \transformer & \msresnet & \tempcnn \\
	\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}
	pre & & & 0.93$^{\pm0.01}$ & 0.93$^{\pm0.01}$ & 0.93$^{\pm0.02}$ & 0.93$^{\pm0.03}$ \\
	raw & & & 0.72$^{\pm0.26}$ & 0.91$^{\pm0.01}$ & 0.88$^{\pm0.02}$ & 0.84$^{\pm0.05}$ \\
	\bottomrule
\end{tabular}

==> tables/preraw2_kappa.tex <==
%\renewcommand{\arraystretch}{.8}
%\setlength\tabcolsep{0pt}
\begin{tabular}{lcccccc}
	\toprule
	kappa & \svm & \rf & \rnn & \transformer & \msresnet & \tempcnn \\
	\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}
	pre & & & 0.88$^{\pm0.01}$ & 0.89$^{\pm0.02}$ & 0.90$^{\pm0.03}$ & 0.88$^{\pm0.05}$ \\
	raw & & & 0.28$^{\pm0.78}$ & 0.84$^{\pm0.02}$ & 0.79$^{\pm0.05}$ & 0.72$^{\pm0.11}$ \\
	\bottomrule
\end{tabular}

==> tables/preraw_accuracy.tex <==
%\renewcommand{\arraystretch}{.8}
%\setlength\tabcolsep{0pt}
\begin{tabular}{lcccccc}
	\toprule
	ov. acc. & \svm & \rf & \rnn & \transformer & \msresnet & \tempcnn \\
	\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}
	preprocessed & & 0.61 & 0.85$^{\pm0.00}$ & 0.87$^{\pm0.01}$ & 0.87$^{\pm0.01}$ & 0.87$^{\pm0.00}$ \\
	raw & & 0.33 & 0.81$^{\pm0.01}$ & 0.82$^{\pm0.02}$ & 0.81$^{\pm0.01}$ & 0.79$^{\pm0.01}$ \\ 
	\bottomrule
\end{tabular}

==> tables/preraw_kappa.tex <==
%\renewcommand{\arraystretch}{.8}
%\setlength\tabcolsep{0pt}
\begin{tabular}{lcccccc}
	\toprule
	kappa & \svm & \rf & \rnn & \transformer & \msresnet & \tempcnn \\
	\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}
	preprocessed & & 0.58 & 0.79$^{\pm0.00}$ & 0.81$^{\pm0.01}$ & 0.82$^{\pm0.02}$ & 0.81$^{\pm0.01}$ \\
	raw & & 0.28 & 0.72$^{\pm0.01}$ & 0.74$^{\pm0.03}$ & 0.72$^{\pm0.01}$ & 0.68$^{\pm0.02}$ \\
	\bottomrule
\end{tabular}
